The XMM-Newton/SDSS Galaxy Cluster Survey (PhD thesis)

The dissertation has been published at the Potsdam University under the following URL: http://opus.kobv.de/ubp/volltexte/2014/7122/

==> Abstract/Ali_Zusammenfassung.tex <==
\chapter{Zusammenfassung}
Im Rahmen dieser Arbeit habe ich die 2XMMi/SDSS Galaxienhaufendurchmusterung erstellt (2XMMi/SDSS galaxy cluster survey), eine Suche nach
Galaxienhaufen welche auf der Detektion ausgedehnter R\"ontgenquellen im XMM-Newton Quellenkatalog (2XMMi-DR3) basiert. Die Hauptziele dieser Suche
sind die Identifizierung bisher unbekannter r\"ontgenheller Galaxienhaufen, die Erforschung deren Verh\"altnisses zwischen R\"ontgenleuchtkraft und
Temperatur (X-ray scaling relation), eine Entdeckung von m\"oglichen weit entfernten Galaxienhaufen und die Beziehung zwischen Eigenschaften im
Optischen und R\"ontgenbereich. Die Durchmusterung ist f\"ur alle Quellen der Himmelsregionen ausgelegt, die vom \emph{Sloan Digital Sky Survey} (SDSS)
erfasst werden. Das Ziel besteht darin ihre optischen Gegenst\"ucke zu finden und deren Rotverschiebungen zu bestimmen. Die gemeinsamen Himmelsareale
zwischen \emph{XMM-Newton} und dem Bildmaterial vom \emph{SDSS-DR7} umfassen \(210 deg^{2}\). Meine Durchmusterung enth\"alt 1180 m\"ogliche
Galaxienhaufen mit wenigstens 80 vom Hintergrund bereinigten Photonen im R\"ontgenbereich, die einer Qualit\"atskontrolle erfolgreich standgehalten
haben.

Um die Rotverschiebungen der m\"oglichen Galaxienhaufen im optischen Bereich zu bestimmen nutzte ich drei Vorgehensweisen: (i) Ein Abgleich jener
Kandidaten mit den neuesten und umfangreichsten Katalogen optisch ausgew\"ahlter Galaxienhaufen, die in der Literatur verf\"ugbar sind. (ii) Ich
entwickelte einen Algorithmus um Rotverschiebungen der optischen Gegenst\"ucke aus Daten vom \emph{SDSS-DR8} zu ermitteln, welches zu photometrischen
Rotverschiebungen von 530 Galaxiengruppen-/haufen f\"uhrte. (iii) Ein weiterer von mir entwickelter Algorithmus nutzte die Rotverschiebung aus Spektren
von roten leuchtkr\"aftigen Galaxien (LRGs) in den Daten des \emph{SDSS-DR9} und ergab 324 Gruppen und Haufen.
Zusammengefasst enth\"alt diese Probe 574 auch im optischen nachgewiesener Galaxiengruppen und -haufen mit bekannten Rotverschiebungen
\(0.03 \lesseq z \lesseq 0.77\) - der zur Zeit umfangreichste Katalog von im R\"ontgenbereich ausgew\"ahlten Galaxienhaufen basierend auf aktuellen
R\"ontgenbeobachtungen. Unter jenen Haufen waren ca. 75\% im R\"ontgenbereich nicht bekannt und 40\% fanden in bisheriger Literatur \"uberhaupt keine
Erw\"ahnung.

Um die R\"ontgeneigenschaften der im Optischen best\"atigten Haufen zu bestimmen, war eine automatische Reduktion und Analyse der R\"ontgendaten
unverzichtbar. Die Prozedur, welche Modelle an die R\"ontgenspektren anpaßte, ergab Temperaturen von \(0.5 - 7.5 keV\) f\"ur 345 Kandidaten. F\"ur alle
Haufen die auch im optischen auffindbar waren, bestimmte ich die physikalischen Eigenschaften \(L_{500} (0.5 \times 10^{42} - 1.2 \times 10^{45} erg~s^{-1}\)
und \(M_{500} (1.1 \times 10^{13} - 4.9 \times 10^{14} M_{\odot}\).

Die Probe optisch best\"atigter Galaxienhaufen mit gemessenen Rotverschiebungen und R\"ontgeneigenschaften kann f\"ur viele astrophysikalische Anwendungen
genutzt werden. Als eine der ersten Anwendungen betrachtete ich die Beziehung zwischen \(L_{X} - T \); das erste Mal f\"ur eine so große Anzahl von
345 Objekten. Der aktuelle Katalog enth\"alt Gruppen und Haufen die einen großen Bereich in Rotverschiebung, Temperatur und Helligkeit abdecken.
Der Anstieg jener Beziehung ist im Einklang mit bereits publizierten Werten f\"ur nahegelegene Galaxienhaufen von hoher Temperatur und Helligkeit.
Nach dem Ausschluuß leuchtschwacher Gruppen und der Einteilung der Daten in drei nach Rotverschiebung geordneter Gruppen waren keine signifikanten
\"Anderungen von Anstieg und intrinsischer Streuung zu beobachten.

Als zweite Anwendung unserer Durchmusterung, untersuchte ich die Haufen bez\"uglich deren Eigenschaften im Optischen und im R\"ontgenbereich. Zuerst
betrachtete ich den Zusammenhang zwischen den Eigenschaften (absolute Helligkeit und optische Leuchkraft) der hellsten Haufengalaxie (BCG) mit denen
des Haufens als Ganzem (Rotverschiebung und Masse). Danach berechnete ich die Reichhaltigkeit der Galaxienhaufen und deren optische Leuchtkraft
innerhalb von \(R_{500}\) f\"ur eine Stichprobe nahegelegener Haufen (\(z \lesseq 0.42\), hier sind SDSS Daten noch empfindlich genug um den Großteil
der Haufengalaxien abzubilden) mit gemessenen R\"ontgentemperaturen. Schlußendlich konnten die Wechselwirkungen zwischen den optischen
Eigenschaften (Reichhaltigkeit und Leuchtkraft) und den globalen Eigenschaften (R\"ontgenleuchtkraft, Temperatur und Masse) n\"aher untersucht werden.


==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 


==> Makefile <==
VERSION=
LATEXTARGET=thesis$(VERSION)

#
# LaTeX Makefile
# --------------
#
# Author : s.m.vandenoord@student.utwente.nl (Stefan van den Oord)
# Date   : March 18, 1999, second version of today.
# 
# This Makefile is a generic makefile for LaTeX documents. Distribute it
# as you wish, but please don't edit or remove this initial comment.
#
# The Makefile can be used by setting the environment variable "MAKEFILES",
# e.g. export MAKEFILES=~/data/TeX/Makefile.
# It requires GNU Make and bash or better, like zsh. Simply sh is not
# sufficient, I believe. The first few lines of the Makefile contains
# the executables that are used, edit them to point to the executables
# on your system.
#
# DISCLAIMER: Using this Makefile is fully at your own risk. I am not
#             responsible for anything! So if crucial files are removed
#             by the Makefile, it is your own problem. But you should
#             have backups anyway. :-)
#
# Usage
# -----
# The Makefile can do the following things for you:
# - generate PostScript equivalents of XFig figures;
# - run makeindex and BibTeX, but only if necessary;
# - compile the .dvi file, running LaTeX as many times as needed;
# - run XDvi with the compiled .dvi file;
# - create a PostScript equivalent of the .dvi file;
# - generate a HTML equivalent of the .dvi file (if Latex2HTML is
#   installed);
# - remove all generated output.
# The Makefile is in some points even RCS aware.
#
# In many cases, you don't even have to tell the Makefile which LaTeX
# file it has to compile. The Makefile uses the following strategy:
# 1. Check if the environment variable LATEXTARGET is set; if it is,
#    generate $LATEXTARGET.dvi.
# 2. If there is only one .tex file, use that one.
# 3. Check if there is a LaTeX file that has the same basename as the
#    directory. For example, if the directory is named "Thesis" and
#    there is a file "Thesis.tex", "Thesis.dvi" is generated.
#
# Invocation
# ----------
# When the MAKEFILES environment variable is set, you can use the
# following commands:
# - make latexhelp
#   Prints an overview of the available commands.
# - make latexfigures
#   Only generate the PostScript equivalents of XFig figures.
# - make file.dvi
#   Generates the specified DVI file.
# - make file.ps
#   Generates the DVI file and then runs dvips.
# - make latex
#   Use the above explained strategy to find out what has to be
#   generated, and generate it.
# - make view
#   Do a make latex and then run XDvi.
# - make latexps
#   Do a make latex and then run dvips.
# - make html
#   Do a make latex and then use LaTeX2HTML to create the HTML equivalent.
#   To do this, the following environment variables are used:
#   * HTMLDIR : the base dir in which the output is written. For example,
#               if HTMLDIR=~/public_html/LaTeX, and the file that is
#               generated is "Thesis", the output will be written in the
#               directory ~/public_html/LaTeX/Thesis.
#   * LATEX2HTML_OPTS : if you want to pass options to LaTeX2HTML, put
#                       them in this variable.
# - make latexclean
#   This command removes all generated output. CAUTION: the files that are
#   removed are thought out pretty well, but it is possible that files are
#   removed that you wanted to keep! Check below what files are removed if
#   you want to be certain!
#   Note that a file figure.eps is only removed if a file figure.fig exists.
#   (Even if the file figure.fig exists, but is checked in using RCS, the
#   file figure.eps will be removed.)
#
# Tip
# ---
# For some projects it is useful to have a separate Makefile in the project's
# directory. For example, when you use RCS, you could add functionality for
# automatic checkouts of the right files (adding dependencies is sufficient;
# GNU Make rocks :-).
# The command "latexclean" is declared so that you can add your own
# functionality in the project's Makefile; instead of one colon, declare it
# with two colons if you want to do that.
# For example:
# latexclean::
#     rm -f foo.bar
# This way both the origional definition in this Makefile and your own are
# used.

#.SILENT:

# SHELL=/usr/local/bin/bash

LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIPS=dvips
MAKEINDEX=makeindex
DVIVIEWER=xdvi -geometry 710x950-0+10
LATEX2HTML=latex2html

FIGURES=$(wildcard *.fig)
FIGUREOBJS=$(FIGURES:.fig=.eps)

TEXFILES=$(wildcard *.tex)

# Disable standard pattern rule:
%.dvi: %.tex

# Do not delete the following targets:
.PRECIOUS: %.aux %.bbl %.eps %.ind

%.aux: %.tex $(FIGUREOBJS) $(TEXFILES)
	@$(LATEX) $*
# Look for citations. Make sure grep never returns an error code.
	@grep "^\\\\citation" *.aux > .btmp.new || true

# If the citations are not changed, don't do anything. Otherwise replace
# the .btmp file to make sure Bibtex will be run.
	@if ( diff .btmp.new .btmp >& /dev/null ); then \
		rm .btmp.new; \
	else \
		mv .btmp.new .btmp; \
	fi

	@if [ -f $*.idx ]; then cp $*.idx .itmp.new; else touch .itmp.new; fi
	@if ( diff .itmp.new .itmp >& /dev/null ); then \
		rm .itmp.new; \
	else \
		mv .itmp.new .itmp; \
	fi

.btmp:

%.bbl: $(BIBFILES) .btmp
# Only use BibTeX if \bibliography occurs in the document. In that case,
# run BibTeX and recompile. .btmp is touched to prevent useless making
# next time.
	@if ( grep "^\\\\bibliography{" $*.tex > /dev/null ); then \
		$(BIBTEX) $*; \
		touch .rerun; \
	fi
	@touch .btmp

.itmp:

%.ind: .itmp
	@if [ -f $*.idx ]; then \
		$(MAKEINDEX) $*; \
		touch .rerun; \
		touch .itmp; \
	fi

%.eps:%.fig
	@echo Generating figure $@...
	@fig2dev -L ps $< $@

%.dvi: %.aux %.ind %.bbl
# Make sure the dvi-file exists; if not: recompile.
	@if [ ! -f $*.dvi ]; then \
		touch .rerun; \
	fi

	@if [ -f .rerun ]; then \
		rm .rerun; \
		$(LATEX) $*; \
	else \
		$(MAKE) $*.aux; \
	fi

# While references et al. are changed: recompile.
	@while ( grep Rerun $*.log > /dev/null ); do \
		$(LATEX) $*; \
	done

# Touch the figureobjects to prevent making next time
	@if [ -n "$(FIGUREOBJS)" ]; then \
		touch $(FIGUREOBJS); \
		touch $*.aux; \
	fi

	@if [ -f $*.ind ]; then \
		touch $*.ind; \
	fi
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo

latex:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

latexfigures:
	@for i in $(FIGUREOBJS); do \
		$(MAKE) $$i; \
	done

view:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi && \
		$(DVIVIEWER) ${LATEXTARGET}.dvi ; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi && \
			$(DVIVIEWER) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi && \
			$(DVIVIEWER) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

%.ps: %.dvi
	$(DVIPS) -o $*.ps $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(DVIPS) -o $*.ps $<

%.pdf: %.tex
	$(PDFLATEX) $<
	@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(BIBTEX) $*
	$(PDFLATEX) $<
	$(PDFLATEX) $<

latexps:
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.ps && \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.ps && \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.ps && \
			true; \
		fi; \
	fi

html: .html

.html:
	@if [ -n "${LATEXTARGET}" ]; then \
		if [ -n "${HTMLDIR}" ]; then \
			$(MAKE) ${LATEXTARGET}.dvi; \
			$(LATEX2HTML) $(LATEX2HTML_OPTS) -dir $(HTMLDIR)/$(LATEXTARGET) $(LATEXTARGET) && \
			chmod a+rx $(HTMLDIR)/$(LATEXTARGET) && \
			chmod a+r $(HTMLDIR)/$(LATEXTARGET)/* &&  \
			touch .html; \
		else \
			echo Set variable HTMLDIR\!; \
		fi; \
	else \
		echo Set variable LATEXTARGET\!; \
	fi

latexhelp:
	@echo "LaTeX Makefile Options"
	@echo "----------------------"
	@echo ""
	@echo "Environment variables:"
	@echo "  LATEXTARGET   Filename to make (without extension)"
	@echo "  HTMLDIR       Directory for HTML-output"
	@echo "  FIGURES       Figures that have to be compiled"
	@echo ""
	@echo "Targets:"
	@echo "  all           Make the LATEXTARGET or <dirname>.dvi"
	@echo "  <name>.dvi    Make the given dvi file"
	@echo "  latex         Make the LATEXTARGET or <dirname>.dvi"
	@echo "  view          Make and view the LATEXTARGET or <dirname>.dvi"
	@echo "  html          Make the LATEXTARGET  or <dirname>.dvi and generate HTML output"
	@echo "  latexhelp     This overview"
	@echo "  latexclean    Remove all generated files"

clean latexclean::
	@rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.out *.brf *.html *.btmp *.itmp *.rerun *.glo *.gls *.nlo *.nls
	@epsfiles=`find * -maxdepth 0  -name "*.eps" `; \
	if [ -n "$$epsfiles" ]; then \
		for i in *.eps; do \
			if [ -f `basename $$i .eps`.fig ]; then \
				rm -f $$i; \
			elif ( rcs `basename $$i .eps`.fig >& /dev/null ); then \
				rm -f $$i; \
			fi \
		done \
	fi

cleanpspdf : clean
	@rm -f *.ps *.pdf

clobber : cleanpspdf
	@rm -f *~

